Doubled Disks and Satellite Surfaces

Conjecturally, a knot is slice if and only if its positive Whitehead double is slice. We consider an analogue of this conjecture for slice disks in the four-ball: two slice disks of a knot are smoothly isotopic if and only if their positive Whitehead doubles are smoothly isotopic. We provide evidence for this conjecture, using a range of techniques. More generally, we consider when isotopy obstructions persist under satellite operations. In particular, we show that obstructions coming from knot Floer homology, Seiberg-Witten theory, and Khovanov homology often behave well under satellite operations. We apply these strategies to give a systematic method for constructing vast numbers of exotic disks in the four-ball, including the first infinite family of pairwise exotic slice disks. These same techniques are then upgraded to produce exotic disks that remain exotic after any prescribed number of internal stabilizations. Finally, we show that the branched double covers of certain stably-exotic disks become diffeomorphic after a single stabilization with $S^2 \times S^2$, hence stabilizing them yields exotic surfaces that have diffeomorphic branched covers.

==> sections/knotfloer.tex <==
\section{Floer Theoretic Background}

\subsection{Knot Floer homology and cobordism maps} \label{sec: knot Floer}

Knot Floer homology, defined in \cite{os_knotinvts} and independently in \cite{rasmussen_knotcompl}, is an invariant of knots, links, and cobordisms between them. In the terminology of \cite{zemke_linkcob}, link Floer homology associates to a decorated link $\mathbf{L}$ a curved complex  $CFL(S^3,\mathbf{L})$ over the commutative ring freely generated over $\mathbb{F}_2$ by formal variables which correspond to basepoints on the decorated link, and to a decorated cobordism a chain map between the curved complexes assigned to its ends. With the aim of being self-contained, we give the definitions of decorated links and cobordisms as well as the category of curved complexes here. For simplicity, we will write ``decorated links'' rather than \emph{multi-based links with a coloring} as in \cite{zemke_linkcob}.

\begin{defn}
A \emph{decorated link} is a 5-tuple $\mathbf{L}=(L,\mathbf{w},\mathbf{z},P,\sigma)$ which satisfies the following conditions.
\begin{itemize}
    \item $L$ is a link in $S^3$.
    \item $\mathbf{w}$ and $\mathbf{z}$ are finite collections of basepoints in $L$, which intersect nontrivially with every component of $L$, such that closures of every component of $L\setminus (\mathbf{w}\cup \mathbf{z})$ has one endpoint in $\mathbf{w}$ and the other endpoint in $\mathbf{z}$.
    \item $P$ is a finite set, and $\sigma$ is a function from $\mathbf{z}\cup\mathbf{w}$ to $P$, which defines a ``coloring'' of the basepoints.
\end{itemize}
\end{defn}

% , for $\mathbf{L}_i = (L_i,\mathbf{z}_i,\mathbf{w}_i,P,\sigma_i)$ with $i=0,1$

\begin{defn}
For $i=0,1$, let $\mathbf{L}_i = (L_i,\mathbf{z}_i,\mathbf{w}_i,P,\sigma_i)$ be decorated links. A \emph{decorated cobordism} between $\mathbf{L}_1$ and $\mathbf{L_2}$ is a 5-tuple $\mathbf{S}=(S,\Sigma_z,\Sigma_w,P,\sigma)$ which satisfies the following conditions.
\begin{itemize}
    \item $S$ is a properly embedded smooth surface in $S^3 \times [0,1]$, such that $\Sigma\cap (S^3 \times \{i\})=L_i$ for $i=0,1$.
    \item $\Sigma_w$ and $\Sigma_z$ are closed subsurfaces of $S$ such that $\Sigma_w \cup \Sigma_z = S$ and $\Sigma_w \cap \Sigma_z$ is a properly embedded 1-dimensional submanifold of $S$.
    \item $L_i \cap \Sigma_w = \mathbf{w}_i$, $L_i \cap \Sigma_z = \mathbf{z}_i$, and $L_i \cap \Sigma_w \cap \mathbf{w}_i$ and $L_i \cap \Sigma_z \cap \mathbf{z}_i$ consist of one point for $i=0,1$.
    \item $\sigma$ is a function from $\pi_0(\Sigma_w) \cup \pi_0(\Sigma_z)$ to $P$, such that every basepoint $p\in \mathbf{w}_i \cup \mathbf{z}_i$ which is contained in a connected component $S\in \pi_0(\Sigma_w)\cup \pi_0(\Sigma_z)$ satisfies $\sigma_i(p)=\sigma(S)$ for $i=0,1$.
\end{itemize}
\end{defn}

Having defined decorated links and cobordisms, we can describe the algebraic structure of knot Floer homology a bit more precisely. Given a finite set $P$, consider the commutative ring $R_P$, freely generated over the field $\mathbb{F}_2$ by the elements of $P$. The curved complex $CFL(S^3,\mathbf{L})$ is a bigraded module over $R_P$. A decorated link cobordism $\mathbf{S}$ between decorated links $\mathbf{L}_1$ and $\mathbf{L}_2$, induces an $R_P$-linear chain map $F_\mathbf{S}$ from $CFL(S^3,\mathbf{L}_1)$ to $CFL(S^3,\mathbf{L}_2)$, which we call the \emph{cobordism map} induced by $\mathbf{S}$.

In this paper, we will focus on knots, i.e. links with only one component (in which case we denote $CFL$ by $CFK$ instead), and concordances between them, i.e. cobordisms between knots which are homeomorphic to cylinders. We can endow a knot $K$ with the simplest possible decoration, consisting of two basepoints $\mathbf{w}=\{w\}$ and $\mathbf{z}=\{z\}$, two colors $P=\{w,z\}$ and the identity coloring function $\mathrm{id}:\{w\}\cup\{z\}\rightarrow \{w,z\}$. In this case, we have $R_P = \mathbb{F}_2[\U,\V]$ where $\U$ and $\V$ are the formal variables associated to the colors $w$ and $z$, and the curvature of the complex $CFK(S^3,\mathbf{K})$ vanishes, so that it becomes a chain complex over $\mathbb{F}_2[\U,\V]$. 

To make expressions simpler, we will abuse notation, and denote both the knot $K$ and the decorated knot $\mathbf{K} = (K, w, z)$ by $K$. We will denote by $CFK^\infty(S^3,K)$ the chain complex over $\mathbb{F}_2[\U,\U^{-1}]$ obtained from $CFK(S^3,K)$ by truncating with $\V=0$ and then localizing by adjoining the formal inverse of $\U$. Furthermore, we denote the truncation of $CFK(S^3,K)$ with $\U=\V=0$ by $\widehat{CFK}(S^3,K)$, and its homology by $\widehat{HFK}(S^3,K)$

In a similar way, a concordance between knots can be endowed with the simplest possible decoration, so $\Sigma_w$ and $\Sigma_z$ are both rectangles. The cobordism map
\[
F_\mathbf{S} : CFK(S^3,K_1)\rightarrow CFK(S^3,K_2),
\]
induced by the decorated cobordism $\mathbf{S}$, is $\mathbb{F}_2[\U,\V]$-linear, bidegree-preserving, and induces a quasi-isomorphism on $CFK^\infty$ by \cite[Theorem C]{zemke_linkcob}.

Again, for simplicity, we will simply write $S$ for the decorated concordance described above. In general, if a decoration is not specified, the chain map $F_S$ is not well-defined up to homotopy; due to the ambiguity induced by full rotations along knots, its homotopy class is defined uniquely only up to composition by the basepoint moving map, which was studied by Sarkar in \cite{sarkar2015moving}, of $K_1$ (or equivalently, $K_2$). However, when either $K_1$ or $K_2$ is unknotted, which is mainly the case that we will be dealing with, then since the basepoint moving map on the unknot is the identity, $F_S$ becomes well-defined up to homotopy (i.e. does not depend on its decoration.)

In particular, if $S$ is the concordance obtained by puncturing a slice disk $D$ of a knot $K$, the chain map
\[
F_S:CFK(S^3, U)\rightarrow CFK(S^3,K)
\]
is well-defined up to homotopy. Truncating by $\U=\V=0$ and then taking homology gives a cobordism map
\[
\widehat{F}_S:\widehat{HFK}(S^3, U)\rightarrow \widehat{HFK}(S^3,K),
\]
which is an invariant of the surface. Since $\widehat{HFK}(S^3, U)\simeq \mathbb{F}_2$, this map can be represented by the homology class
\[
t_D \coloneqq \hat{F}_S(1) \in \widehat{HFK}(S^3,K).
\]
Note that the class $t_D$ depends only on the smooth isotopy class of the given slice disk $D$. This fact was first observed in \cite{juhasz2016concordance}.

\subsection{Bordered Floer homology}\label{sec: bordered backgroun}



Bordered Floer homology is a package of invariants of 3-manifolds with parametrized boundary. Bordered Floer homology associates to a surface $F$ a differential graded algebra $\cA(F)$ and to a 3-manifold $Y$ with boundary together with an identification $\vphi: \partial Y \ra F$ a left differential graded module over $\cA(-F)$, called $\CFDh(Y)$ and a right $\cA_\infty$-module over $\cA(F)$ called $\CFAh(Y)$.

Bordered Floer homology has a pairing theorem \cite[Theorem 1.3]{LOT_bordered_HF}, which recovers the hat-version of the Heegaard Floer homology of the manifold obtained by gluing bordered manifolds along their common boundary. Given 3-manifolds $Y_1$ and $Y_2$ with $\partial Y_1 \cong F \cong \partial Y_2$, there is a homotopy equivalence
\[
	\CFh(Y_1\cup Y_2) \simeq \CFAh(Y_1) \boxtimes_{\cA(F)} \CFDh(Y_2).
\]
Bordered Floer theory also recovers knot Floer homology \cite[Theorem 11.21]{LOT_bordered_HF}. Given a doubly pointed bordered Heegaard diagram $(\mathcal{H}_1, w, z)$ for $(Y_1, \partial F, K)$ and a bordered Heegaard diagram $(\mathcal{H}_2, z)$ with $\partial Y_1 \cong F \cong -\partial Y_2$, then 
\[
	\HFKh(Y_1 \cup Y_2, K) \cong H_*(\CFAh(\mathcal{H}_1, w, z) \boxtimes_{\cA(F)} \CFDh(\mathcal{H}_2, z)).
\]
Bordered Floer theory, therefore, gives an effective way to study satellites. If $P(K)$ is the satellite of $K$ with pattern $P$, then $\HFKh(S^3, P(K))$ can be computed by finding a doubly pointed bordered Heegaard diagram $\mathcal{H}_P$ for the pattern $P$ in the solid torus and computing the box tensor product $\CFAh(\mathcal{H}_P) \boxtimes \CFDh(S^3 \smallsetminus K)$. \\

Much in the same way, by passing through bordered Floer homology, we can compute link cobordism maps associated to satellite concordance in terms of the  maps associated to the original concordance.

\begin{theorem}{\cite[Theorem 2]{guth_one_not_enough_exotic_surfaces}}\label{Theorem: satellite formula for concordance maps}
    Let $C: K \ra K'$ be a smooth concordance. Then, there exists a map $F: \CFDh(S^3 \smallsetminus K) \ra \CFDh(S^3 \smallsetminus K')$ induced by $C$, such that for any pattern knot $P$ in the solid torus and a suitable decoration on $P(C)$, the following diagram commutes up to homotopy:

    \begin{center}
        \begin{tikzcd}
            \CFAh(\mathcal{H}_P) \boxtimes \CFDh(S^3 \smallsetminus K) \ar[d, "\bI_{\CFAh(\mathcal{H}_P)} \boxtimes F"]  \ar[r, "\simeq"]  
                & \CFKh(S^3, P(K)) \ar[d, "F_{P(C)}"]  \\
            \CFAh(\mathcal{H}_P) \boxtimes \CFDh(S^3 \smallsetminus K') \ar[r, "\simeq"]
                & \CFKh(S^3, P(K^\prime)),
        \end{tikzcd}
    \end{center}
where $\mathcal{H}_P$ is a doubly pointed, bordered Heegaard diagram for $P\sub S^1\times D^2$, $P(K)$ and $P(K^{\prime})$ are satellites of $K$ and $K^{\prime}$, and $P(C)$ is the satellite concordance induced by $P$. The horizontal arrows are given by the pairing theorem \cite{LOT_bordered_HF}. 
\end{theorem}
\section{Disk maps and knot doubling operators}\label{sec: disk maps and doubling}

In this section we prove the key proposition which will lead to the proof of \Cref{thm:1}. 

\begin{prop}\label{prop: doubled invariants}
Let $K$ be a knot in $S^3$ and let $D_1$ and $D_2$ be a pair of slice disks for $K$. If the invariants $t_{D_1}$ and $t_{D_2}$ are distinct in $\HFKh(S^3, K)$, then for any knot $J$ and $s < 2\tau(J)$, $t_{\Lev_{J, s}(D_1)}$ and $t_{\Lev_{J,s}(D_2)}$ are distinct as well. 

%\footnote{\GG{We could generalize this? Our proof just uses the fact that the type-A module associated to the pattern has no operations of the form: $m_k(a, ...) = a$, where $a$ is the generator which survives after tensoring with the type-D module for the unknot complement. Both the doubling and cabling patterns have this property.} \SK{I totally agree.}}
\end{prop} 

In fact, we give a simple criterion for determining when an unknotted pattern $P$ is guaranteed to produce $\HFKh$-distinguishable disks, in terms of the structure of $\CFAh(S^1\times D^2, P)$. 

When $P$ is an unknotted pattern, 
\[
\CFAh(S^1\times D^2, P) \boxtimes \CFDh(S^3-U) \simeq \CFKh(S^3, U).
\]
Therefore, there is some element $a$ in $\CFAh(S^1\times D^2, P)$ such that $a \otimes v$ generates homology of $\CFKh(S^3, U)$, where $v$ is the unique element in $\CFDh(S^3\setminus U)$. On homology, $\bI_P \boxtimes F$ is therefore determined by the image of $a\otimes v$. We show that given some seemingly restrictive assumptions on the structure of $\CFAh(S^1\times D^2, P)$, $\bI_P \boxtimes F$ is guaranteed to be nontrivial on homology. 

\begin{lemma}\label{lem: no cancellation} \footnote{\GG{Tying out proving the ``no cancellation'' lemma first. This seemed cleaner, since we end up showing lots of patterns have this property.}}
Let
\[
F: \CFDh(S^3\setminus U) \ra \CFDh(S^3 \setminus K),
\]
be a morphism of type-D structures which tensors with the identity map of $\CFAh(S^1\times D^2, \lambda)$ to give a nontrivial map, where $\lambda$ is the knot $S^1 \times \pt \sub S^1 \times D^2$. Let $a$ be an element of $\CFAh(S^1 \times D^2, P)$ such that $a \otimes v$ generates the homology of $\CFAh(S^1 \times D^2, P)\boxtimes \CFDh(S^3\setminus U)$ and extend $\{a\}$ to a basis for $\CFAh(S^1 \times D^2, P)$. If the coefficient of $a$ is zero in every $\cA_\infty$ operation $m_k(b, \rho_{i_1}, \hdots, \rho_{i_{k-1}}) $ of $\CFAh(S^1 \times D^2, P)$ which preserves the filtration, then the map 
\[\bI_P \boxtimes F: H_*(\CFAh(S^1 \times D^2, P)\boxtimes \CFDh(S^3\setminus U)) \ra H_*(\CFAh(S^1 \times D^2, P)\boxtimes \CFDh(S^3\setminus K))\] 
is nontrivial.
\end{lemma}
\begin{proof}
Let $x = F(v)$, where $F$ is the map of type-D structures induced by $F_C$. We can write 
\[
x = 1\cdot \theta + \sum_{I \in \{1, 2, 3, 12, 23, 123\}} \rho_I \theta_I,
\]
for some $\theta_I \in\CFDh(S^3\setminus K)$. The term $\theta$ must be nontrivial, since we have assumed that  $\bI_{\CFAh(S^1\times D^2, \lambda)} \boxtimes F$ has nontrivial image (this follows from the fact that $\CFAh(S^1\times D^2, \lambda)$ has no nontrivial $\cA_\infty$-operations and so all other terms in $F(x)$ are annihilated after taking the box tensor product.) $(\bI_P \boxtimes F)(a\otimes v)$ is defined to be
\begin{align*}
(\bI_P \boxtimes F)(a\otimes v) &= \sum_{k=1}^\infty (m_{k+1}\otimes \bI_P) \circ (a \otimes F^k(v))\\
&= a \otimes \theta + \text{ other terms}.
\end{align*}
The term $a\otimes \theta$ could be canceled if, for some $k$, $F^k(v)  = \rho_{i_1}\otimes \hdots\otimes \rho_{i_k} \otimes \theta$ and there is an operation of the form $m_{k+1}(a, \rho_{i_1}, \hdots, \rho_{i_k})$ in which $a$ appears with nonzero coefficient. However, we have assumed that no such operations exist. 

Moreover, when we pass to homology, there are no relations between $a\otimes \theta$ and any other elements of $H_*(\CFAh(S^1 \times D^2, P)\boxtimes \CFDh(S^3\setminus K))$, since $a\otimes \theta$ could only appear as a term in the boundary of another element if there were a filtration preserving operation of the form $m_{k+1}(b, \rho_{i_1}, \hdots, \rho_{i_k})$ in which $a$ appeared with nonzero coefficient. Again, no such operations exist. 

Therefore, $a \otimes \theta$ appears as a non-canceling term in the expansion of $(\bI_P \boxtimes F)(a\otimes v) \in H_*(\CFAh(S^1 \times D^2, P)\boxtimes \CFDh(S^3-K))$, from which it follows that $\bI_P \boxtimes F$ has nontrivial image.
\end{proof}

Therefore, it suffices to show that Levine's satellites patterns satisfy the hypotheses of Lemma \ref{lem: no cancellation}.\\

We begin with some setup, following \cite{levine_doubling_operators}. As described in \cite[Chapter 11]{LOT_bordered_HF}, the type-D structure for the zero-framed complement of $K$,  $\CFDh(S^3 \smallsetminus K)$ is determined by $\CFK^\infty(S^3,K)$. First, fix two simple bases for $\CFK^\infty(S^3,K)$: a vertically simplified basis $\xi_0, \hdots, \xi_{2n}$ with vertical arrows $\xi_{2j-1} \to \xi_{2j}$ of length $k_j$ as well as a horizontally simplified basis $\eta_0, \hdots, \eta_{2n}$ with horizontal arrows $\eta_{2j-1} \to \eta_{2j}$ of length $\ell_j$. Let $(x_{ij})$ be the change of basis matrix. 

The type-D structure $\CFDh(S^3 \smallsetminus K)$ can then be described as follows: $\iota_0 \cdot \CFDh(S^3 \smallsetminus K)$ inherits two bases, which by abuse of notation, we denote $\xi_0, \hdots, \xi_{2n}$ and $\eta_0, \hdots, \eta_{2n}$, which are related by the matrix $(x_{ij})$; $\iota_1 \cdot \CFDh(S^3 \smallsetminus K)$ has a basis 
\[\bigcup_{j=1}^n\{\kappa_1^j, \hdots, \kappa_{k_j}^j\}\cup \{\lambda_1^j, \hdots, \lambda^j_{\ell_j}\}.\]
For each arrow vertical $\xi_{2j-1} \to \xi_{2j}$ of $\CFK^\infty(S^3,K)$, $\CFDh(S^3 \smallsetminus K)$ has differentials
\[
    \xi_{2j}\xra{\rho_{123}} \kappa_1^j \xra{\rho_{23}} \hdots \xra{\rho_{23}} \kappa_{k_j}^j \xleftarrow{\rho_{1}}\xi_{2j-1}
\]
and for each horizontal arrow $\eta_{2j-1} \to \eta_{2j}$, $\CFDh(S^3 \smallsetminus K)$ has differentials
\[
    \eta_{2j-1}\xra{\rho_{3}} \lambda_1^j \xra{\rho_{23}} \hdots \xra{\rho_{23}} \lambda_{\ell_j}^j \xra{\rho_{2}}\eta_{2j-1}.
\]
The summands of $\CFDh(S^3 \smallsetminus K)$ generated by the $\xi_i$ and $\eta_i$ are usually called stable chains. There is one final summand, typically called the unstable chain, which depends on the framing and $\tau(K)$. However, since we will be working with zero-framed slice knots the unstable chain is quite simple:
\[
\eta_0 \xleftarrow{\rho_{12}} \xi_0.
\]

The type-A structure associated to the pattern $\Lev_{J, s}$ in the solid torus, which we denote $\CFAh(S^1 \times D^2,\Lev_{J, s})$, is computed by Levine. As the knot $J$ is unspecified, the computation is quite complicated. We will only need to consider a small subset of the $\cA_\infty$-operations, so we will only provide a terse description of this module, and refer the careful reader to \cite[Section 3]{levine_doubling_operators}. 

When $s < 2\tau(J)$, the type-A structure $\CFAh(S^1 \times D^2,\Lev_{J, s})$ is generated by elements 
\[
    A^j, A'^j, B^j, B'^j, C^j, C'^j, D^j, D'^j, E^j_i, E'^j_i, F^j_i, F'^j_i, G^j_i, G'^j_i, H^j_i, H'^j_i, 
\]
where $0 \le j \le \text{rank}(\iota_0 \cdot \CFDh(S^3 \smallsetminus J))$ and $1 \le i \le k_j$, where $k_j$ is the length of the arrow between the $(2j-1)^{th}$ and $(2j)^{th}$ generators of $\iota_0 \cdot \CFDh(S^3 \smallsetminus J)$.

In this case (where $s < 2\tau(J)$), Levine shows that the homology of  $\CFAh(S^1 \times D^2,\Lev_{J, s}) \boxtimes \CFDh(S^3 \smallsetminus U)$ is generated by $A^0 \otimes v$, where $v$ is the single generator of $\CFDh(S^3 \smallsetminus U).$ Since we are only interested in the image of this element under the maps induced by the doubles of the disks in consideration, it suffices to consider those $\cA_\infty$-operations involving $A^0$, and since we are only interested in computing $\HFKh$, we need only consider those arrows in and out of $A^0$ which preserve the filtration:
\begin{align*}
    m_2(A^0, \rho_1) & =  B^0  \\
    m_2(A^0, \rho_{12}) &= G^0_1 
\end{align*}
Therefore, all criteria of Lemma \ref{lem: no cancellation} are satisfies, so Proposition \Cref{prop: doubled invariants} follows.
\begin{comment}

\begin{proof}[Proof of \Cref{prop: doubled invariants}]
By assumption,
\[
    t_{D_1} + t_{D_2} \ne 0 \in \HFKh(S^3, K).
\]
By \Cref{Theorem: satellite formula for concordance maps}, the maps $F_{D_1}$ and $F_{D_2}$ induce corresponding maps \[f_1, f_2: \CFDh(S^3 \smallsetminus U) \ra \CFDh(S^3 \smallsetminus K)\] which compute the maps associated to satellites of $D_1$ and $D_2$.  Let $x = f_1(v) + f_2(v)$, where $v$ is the single generator of $\CFDh(S^3 \smallsetminus U)$.

Write $x$ as a linear combination
\[
    x = \theta + \sum_{J \in \{1, 2, 3, 12, 23, 123\}} \rho_J \theta_J,
\]
where $\theta$ is a sum of basis elements with algebra coefficient 1. Let $\CFAh(S^1\times D^2, \lambda)$ be the type-A structure associated to the longitudinal unknot in the solid torus. This module has a single generator $\alpha$ and a single nontrivial $\cA_\infty$-operation, $m_2(\alpha, 1) = \alpha$. Again, by \Cref{Theorem: satellite formula for concordance maps}, \[\bI_{\CFAh(S^1\times D^2, \lambda)}\boxtimes (f_1 + f_2) \simeq F_{D_1} + F_{D_2}.\] For this map to be nonzero, it must be that $\theta$ is nonzero, as none of the other terms in the expansion of $x$ survive after taking the tensor product with $\bI_{\CFAh(S^1\times D^2, \lambda)}$. It then follows that $A^0\otimes \theta$  must appear as a term in $(\bI_{\CFAh(S^1 \times D^2,\Lev_{J,s})}\boxtimes (f_1 + f_2))(A^0 \otimes x)$. To prove that this map is nonzero, it suffices to show that, in homology, this term cannot be canceled by any other terms which appear in $(\bI_{\CFAh(S^1 \times D^2,\Lev_{J,s})}\boxtimes (f_1 + f_2))(A^0 \otimes x)$.

By definition, terms appearing in $(\bI_{\CFAh(S^1\times D^2, \Lev_{J,s})}\boxtimes (f_1 + f_2))(A^0 \otimes x)$ are of the form $(m_{k+1} \otimes \bI) \circ (A^0\otimes (f_1 + f_2)^k(x))$. Hence the term $A^0 \otimes \theta$ appears. This term could only be canceled at the chain level if there were an element $y \in \CFDh(S^3 \smallsetminus K)$ so $\delta^k(y) = \alpha_1 \otimes \hdots \alpha_k \otimes \theta$ and $m_{k+1}(A^0, \alpha_1, \hdots, \alpha_k) = A^0.$ However, there are no such $\cA_\infty$ operations. Moreover, for the same reason, $A^0 \otimes \theta$ persists in homology, as there are no $A_\infty$ operation of the form $m_{k+1}(X,\alpha_1,\cdots,\alpha_k)=A^0$, so $A^0 \otimes \theta$ cannot appear in the boundary of any other element of $\CFAh(S^1 \times D^2,\Lev_{J, s})\boxtimes \CFDh(S^3\smallsetminus K)$.

Hence the term $A^0 \otimes \theta$ can never be canceled, and therefore the quantity
\[
t_{\Lev_{J,s}(D_1)}+t_{\Lev_{J,s}(D_2)} = [(\bI_{\CFAh(S^1\times D^2, \Lev_{J,s})}\boxtimes (f_1 + f_2))(A^0 \otimes x)]
\]
is nonzero in $\HFKh(S^3, \Lev_{J,s}(K))$, as desired.
\end{proof}
\end{comment}


\begin{comment}
Now we are able to prove \Cref{thm:1}.
\begin{proof}[Proof of \Cref{thm:1}]
It follows from the satellite formula for Alexander polynomials that for any knot $K$, the doubled knot $\Lev_{J,s}(K)$ has Alexander polynomial 1. Since $\Lev_{J,s}(D_1)$ and $\Lev_{J,s}(D_2)$ are $\Z$-disks, it follows from \cite[Theorem 1.2]{conway2021embedded} that they are topologically isotopic. On the other hand, it follows from \Cref{lem: doubled invariants} that they cannot be smoothly isotopic rel.\ boundary.
\end{proof}
\end{comment}


\subsection{Disks distinguished by knot Floer homology}

From \Cref{thm:1}, we see that to construct exotic disks bounding $\Lev_{J,s}(K)$, it suffices to construct two slice disks of $K$ which are distinguished by their induced maps on knot Floer homology. It is very easy to find such examples; a systematic way of finding them comes from a 4-dimensional construction called \emph{deformation-spinning}, which we will now define.

\begin{defn}\label{def:spinning}
Let $a$ be a properly embedded smooth arc in $D^3$.
  Furthermore, let $\phi \colon I \times D^3 \to D^3$ be an isotopy of $D^3$ such that
  $\phi_0 = \mathrm{id}_{D^3}$, $\phi_t \vert_{\partial D^3} = \mathrm{id}_{\partial D^3}$ for every $t \in I$, and $\phi_1(a) = a$.
  Then the \emph{deform-spun} slice disk $D_{a, \phi} \subset D^4$ is defined by taking
  \[
  \bigcup_{t \in I} \{t\} \times \phi_t(a) \subset I \times D^3,
  \]
  and rounding the corners along $\{0, 1\} \times \partial D^3$.
  When the arc $a$ is understood, we simply write $D_{\phi}$ instead of $D_{a, \phi}$.
\end{defn}

It was observed in \cite[Lemma 3.3]{juhász_zemke_dist_slice_disks} that given an (orientation-preserving) self-diffeomorphism $d$ of $(D^3, a)$ such that $d|_{\partial D^3} = \mathrm{id}_{\partial D^3}$, there exists an isotopy $\phi \colon I \times D^3 \to D^3$, such that $\phi_1 = d$. Furthermore, the isotopy class of the deform-spun disk $D_{a, \phi}$ only depends on $d$. Hence we will denote $D_{a,\phi}$ by $D_{a, d}$ for simplicity.

\begin{defn}\label{def: deform spun}
Let $K$ be a knot in $S^3$, and suppose that the open 3-ball $B$ intersects $K$ in an unknotted arc.
Then $(S^3 \smallsetminus B, K \smallsetminus B)$ is diffeomorphic to a ball-arc pair $(D^3, a)$.
Suppose that we are given a diffeomorphism $d \in \mathrm{Diff}(S^3, K)$ that is the identity on $B$.
Then the \emph{deform-spun} slice disk $D_{K, d} \subset B^4$ for $-K \# K$ is defined
to be $D_{a, d|_{S^3 \smallsetminus B}}$.
\end{defn}

Now we are able to prove \Cref{cor:1}.

\begin{proof}[Proof of \Cref{cor:1}]
Consider the diffeomorphism $R^\pi:(S^3,K\# K)\rightarrow (S^3,K\# K)$ which swaps the two summands of $K\# K$ as in \Cref{fig:KsharpK}. The action of $R^\pi$ on $\widehat{HFK}(S^3,K\# K)$ (or more generally, $HFK^\infty(S^3,K)$) was identified in \cite[Theorem 8.1]{juhasz_zemke_stabilization_bounds} as
\[
(R^\pi)_\ast = \mathrm{Sw}\circ (1\otimes (1+\Psi\Phi) + \Psi\otimes \Phi),
\]
where $\mathrm{Sw}$ denotes the automorphism of the group
\[
\widehat{HFK}(S^3,K\# K)\simeq \widehat{HFK}(S^3,K)\otimes \widehat{HF}(S^3,K)
\]
which switches the two $\widehat{HFK}(S^3,K)$ factors.

\begin{figure}[h]
    \centering
    \includegraphics[scale=.4]{figures/swapdiff2.pdf}
    \caption{The knot $K\# K$, when $K$ is the figure-eight knot in this figure. The diffeomorphism $R^\pi$ acts by rotation along the dotted axis.}
    \label{fig:KsharpK}
\end{figure}

Choose any nonzero element $a_0\in \widehat{HFK}(S^3,K)$. If $\Phi(a_0)=0$, then we define $a=a_0$; otherwise we take $a=\Phi(a_0)$, so that $\Phi(a)=\Phi^2(a_0)=0$ since $\Phi^2=0$ \cite[Lemma 4.9]{zemke2019link}. Since the hat version of knot Floer homology detects the unknot \cite{os_genusbounds}, we can find a nonzero element $b\in \widehat{HFK}(S^3,K)$ which is different from $a$. Then we have
\[
(R^\pi)_\ast(b\otimes a) = \mathrm{Sw}(b\otimes a) = a\otimes b.
\]
Since $a\ne b$ and $a,b$ are both nonzero, we see that $(R^\pi)_\ast$ is not homotopic to the identity. From \cite[Theorem 5.1]{juhász_zemke_dist_slice_disks}, we then see that the deform-spun slice disks $D_{K\# K,R^\pi}$ and $D_{K\# K,\mathrm{id}}$ of $K\# K\# -K\# -K$, induced by the diffeomorphisms $R^\pi$ and $\mathrm{id}$, satisfy $t_{D_{K\# K,R^\pi}} \ne t_{D_{K\# K,\mathrm{id}}}$ in $\widehat{HFK}(S^3,K\# K\# -K\# -K)$. Therefore, by \Cref{thm:1}, the slice disks $\Lev_{J,s}(D_{K\# K,R^\pi})$ and $\Lev_{J,s}(D_{K\# K,\mathrm{id}})$ are topologically isotopic but not smoothly isotopic.
\end{proof}

\subsection{Cables and Stabilization Distance}

We will now use the same strategy to prove \Cref{thm:1-1}. Recall from \cite{homcabling} that the type-A structure $CFA^-(S^1 \times D^2,C_{p,1})$, where $C_{p,1}$ denotes the $(p,1)$-cabling pattern in the $\infty$-framed solid torus for $p\ge 1$, is generated by $a,b_1,\cdots,b_{2p-2}$, where the $A_\infty$ operations are given as follows.
\[
\begin{split}
    m_{3+i}(a,\rho_3,\overbrace{\rho_{23},\cdots,\rho_{23}}^{i},\rho_2) = U^{pi+p} a, &\quad i\ge 0, \\
    m_{4+i+j}(a,\rho_3,\overbrace{\rho_{23},\cdots,\rho_{23}}^{i},\rho_2,\overbrace{\rho_{12},\cdots,\rho_{12}}^{j},\rho_1) = U^{pi+j+1} b_{j+1}, &\quad 0\le j\le p-2,\,i\ge 0, \\
    m_{2+j} (a,\overbrace{\rho_{12},\cdots,\rho_{12}}^{j},\rho_1) = b_{2p-j-2}, &\quad 0 \le j \le p-2, \\
    m_1 (b_j) = U^{p-j} b_{2p-j-1}, &\quad 1 \le j \le p-1, \\
    m_{3+i} (b_j,\rho_2,\overbrace{\rho_{12},\cdots,\rho_{12}}^{i},\rho_1) = U^{i+1}b_{j+i+1}, &\quad 1 \le j \le p-2, \, 0 \le i\le p-j-2, \\
    m_{3+i} (b_j,\rho_2,\overbrace{\rho_{12},\cdots,\rho_{12}}^{i},\rho_1) = b_{j-i-1}, &\quad p+1 \le j \le 2p-2, \, 0 \le i \le j-p-1.
\end{split}
\]
Note that we have the following pairing formula for any knot $K$:
\[
CFK^-(S^3,K) \simeq CFA^-(S^1 \times D^2,C_{p,1}) \boxtimes \widehat{CFD}(S^3 \setminus K).
\]

\begin{proof}[Proof of \Cref{thm:1-1}]
By \Cref{Theorem: satellite formula for concordance maps}, we have two type-D morphisms
\[
f_1,f_2:\widehat{CFD}(S^3 \setminus U)\rightarrow \widehat{CFD}(S^3 \setminus K)
\]
which compute the maps associated to satellites of $D_1$ and $D_2$. Let $x=f_1(v)+f_2(v)$, where $v$ is the single generator of $\widehat{CFD}(S^3 \setminus U)$, and write 
\[
x = \theta + \sum_{J\in \{1,2,3,12,23,123\}} \rho_J \theta_J,
\]
as in the proof of \Cref{lem: doubled invariants}. Since $t_{D_1}+t_{D_2}\ne 0$ in $\widehat{HFK}(S^3,K)$, we know that $\theta$ is nonzero. Since the homology of the chain complex
\[
\mathbb{F}_2[U] \simeq CFK^-(S^3,U)\simeq CFA^-(S^1 \times D^2,C_{p,1})\boxtimes \widehat{CFD}(S^3 \setminus U)
\]
is generated by $a\otimes v$, we know that $t_{(D_1)_{p,1}} + t_{(D_2)_{p,1}}$ is the homology class of
\[
(\mathrm{id}_{CFA^-(S^1 \times D^2,C_{p,1})}\boxtimes (f_1+f_2))(a \otimes v),
\]
which contains the term $a \otimes \theta$. Since any $A_\infty$ operation in $CFA^-(S^1 \times D^2,C_{p,1})$ which has some $\mathbb{F}_2[U]$-multiple of $a$ as an output has coefficients of the form $U^{pi+p}$ for some $i\ge 0$, it is clear from the no-cancellation argument used in the proof of \Cref{lem: doubled invariants} that $U^k (t_{(D_1)_{p,1}} + t_{(D_2)_{p,1}})$ is nonvanishing in homology whenever $0 \le k < p$. It then follows from \cite[Theorem 1.1]{juhasz_zemke_stabilization_bounds} that the stabilization distance between $(D_1)_{p,1}$ and $(D_2)_{p,1}$ is at least $p$.

\SK{
\begin{rem}
One can use the same argument, using the computation of type-A module $CFA^-(T_\infty,M)$ in \cite[Figure 3]{petkova2021twisted}, where $M$ denotes the Mazur pattern, to prove the following: for any disks $D_1,D_2$ with $t_{D_1}\neq t_{D_2}$, we have $t_{M(D_1)}\neq t_{M(D_2)}$.
\end{rem}
}
\end{proof}
